Improving incremental signature-based Groebner basis algorithms

In this paper we describe a combination of ideas to improve incremental signature-based Groebner basis algorithms having a big impact on their performance. Besides explaining how to combine already known optimizations to achieve more efficient algorithms, we compare the quite different effects on the two best-known algorithms in this area, F5 and G2V, both from a theoretical and a practical point of view.

==> layout.tex <==
% Index style
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% indent of subitems only 10pt ( 20pt is standard )
\makeatletter
  \renewcommand*\subitem{\@idxitem \makebox[10pt][r]{}}
\makeatother


% Bibliography style
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibliographystyle{acm}


% ALGORITHM style
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

% Header style
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\clearscrheadfoot 
%\automark[section]{section}
\chead{\small{\headmark}} 
\ohead[\pagemark]{\pagemark} 
\setheadwidth[0pt]{\dimexpr \textwidth} 

\renewcommand*{\chapterpagestyle}{empty}
% package sectsty
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\chapterfont{}
%\sectionfont{}
%\subsectionfont{}


% TOC-LOT-LOF-LOA style
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\renewcommand{\cfttoctitlefont}{\Large\bfseries\sc}
%\renewcommand{\cftlottitlefont}{\Large\sc}
%\renewcommand{\cftloftitlefont}{\Large\sc}
%\renewcommand{\cftpartfont}{\large\sc}
%\renewcommand{\cftchapfont}{\sc}
%\renewcommand{\cftsecfont}{\small\sc}


% Par style
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\parskip 
\parindent 3ex


% Itemize elements
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand\labelitemi{$\triangleright$} % dreieck statt punkt 


% Nummerierungsart ändern??
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand {\labelenumi}{(\arabic {enumi})}
\renewcommand {\theenumi}{(\arabic {enumi})}
%\renewcommand {\labelenumii}{(\roman {enumii})}
%\renewcommand {\theenumii}{(\roman {enumii})}

%\renewcommand{\thepart}{\Roman{part}}
%\renewcommand{\thechapter}{\arabic{chapter}}
%\renewcommand{\thesection}{\thechapter.\arabic{section}}
%\renewcommand{\thesubsection}{\thesection.\arabic{subsection}}

% package titlesec
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\titleformat{\part}%
  {\bfseries\sc\Huge\centering}{\thepart}{1.0em}{\thispagestyle{empty}}
\titleformat{\chapter}%
  {\bfseries\sc\huge\centering}{\thechapter}{1.0em}{}
\titlespacing{\chapter}
             {0em}{20em}{10em}[0em]
\titleformat{\section}%
  {\bfseries\Large\centering}{\thesection}{1.0em}{\sc}
\titlespacing{\section}
             {0em}{5em}{2em}[0em]
\titleformat{\subsection}%
  {\bfseries\centering}{\thesubsection}{1.0em}{\sc}


==> nocites.tex <==
\nocite{singular313}
\nocite{gpSingularBook2007}

